A Novel Control Strategy for Offset Points Tracking in the Context of Agricultural Robotics

In this paper, we present a novel method to control a rigidly connected location on the vehicle, such as a point on the implement in case of agricultural tasks. Agricultural robots are transforming modern farming by enabling precise and efficient operations, replacing humans in arduous tasks while reducing the use of chemicals. Traditionnaly, path_following algorithms are designed to guide the vehicle's center along a predefined trajetory. However, since the actual agronomic task is performed by the implement, it is essential to control a specific point on the implement itself rather than vehicle's center. As such, we present in this paper two approaches for achieving the control of an offset point on the robot. The first approach adapts existing control laws, initially inteded for rear axle's midpoint, to manage the desired lateral deviation. The second approach employs backstepping control techniques to create a control law that directly targets the implement. We conduct real-world experiments, highlighting the limitations of traditional approaches for offset points control, and demonstrating the strengths and weaknesses of the proposed methods.

==> kinematic_model.tex <==
\begin{tikzpicture}
\begin{scope}
    \def \Xpathcenter{0};
    \def \Ypathcenter{0};
    \def \Rpath{5};
    \def \angle{35};
    \def \y{\Rpath/4};
    \def \Ts{3};
    \def \Ty{0.75}
    \def \thetatilde{15}
    \def \deltac{20}
    \def \wheelheight{0.1125}
    \def \wheelwidth{0.515625}
    \def \wheelbase{2.5}
    \coordinate (Origin) at (0,0);
    \coordinate (O) at (0,{\Rpath+\y});
    \coordinate (S) at (0,{\Rpath});
    \coordinate (F) at ({\wheelbase*cos(\thetatilde)},{\Rpath+\y-\wheelbase*sin(\thetatilde)});
    \coordinate (F1) at ({(\wheelbase+1.5)*cos(\thetatilde)},{\Rpath+\y-(\wheelbase+1.5)*sin(\thetatilde)});
    \coordinate (M) at ({-\Ts*cos(\thetatilde)}, {\Rpath+\y +\Ts *sin(\thetatilde)});
    \def \xT{{-\Ts*cos(\thetatilde)+\Ty*sin(\thetatilde)}}:
    \def \yT{{\Rpath+\y +\Ts *sin(\thetatilde)+\Ty*cos(\thetatilde)}}
    \coordinate (T) at (\xT,\yT);
    
    
    \draw[black,thick,name path=trajectory, domain=90-\angle:90+\angle] plot ({\Xpathcenter+\Rpath*cos(\x)}, {\Ypathcenter+\Rpath*sin(\x)}) 
    ({\Rpath*sin(\angle) -0.5}, {\Rpath}) node[below] {$\Gamma$};

    \draw[line width=0.5mm, RoyalPurple] (O) -- (F);

    \draw[line width=0.5mm, RoyalPurple] (O) -- (M) node[midway, above, black] {$T_s$};
    
    \draw[line width=0.5mm, RoyalPurple] (M) -- (T) node[below left, black] {$T_y$} ;

    \filldraw[Purple] (T)  node[above left, black] {$T$} circle(4pt) ;
    
    \filldraw[rounded corners,Purple,rotate around={-\thetatilde:(O)}] (-\wheelwidth,{\Rpath+\y-\wheelheight}) rectangle (\wheelwidth,{\Rpath+\y+\wheelheight});
    
    \filldraw[rounded corners,Purple,rotate around={{-\thetatilde - \deltac}:(F)}] ({\wheelbase*cos(\thetatilde)-\wheelwidth}, {\Rpath+\y-\wheelbase*sin(\thetatilde)-\wheelheight}) rectangle ({\wheelbase*cos(\thetatilde)+\wheelwidth},{\Rpath+\y-\wheelbase*sin(\thetatilde)+\wheelheight});

    \draw [-stealth,line width=0.5mm, red](O) -- ++(1,0);

    \draw [-stealth,line width=0.5mm, red, rotate around={{-\thetatilde - \deltac}:(F)} ](F) -- ({\wheelbase*cos(\thetatilde)+1},{\Rpath+\y-\wheelbase*sin(\thetatilde)});

   \draw [-stealth,line width=0.5mm, OliveGreen, rotate around={\thetatilde:(T)}](T) -- ({-\Ts*cos(\thetatilde)+\Ty*sin(\thetatilde)+1}, {\Rpath+\y +\Ts *sin(\thetatilde)+\Ty*cos(\thetatilde)});

    \draw[densely dotted] (-{\Rpath*sin(\angle)-0.5}, \Rpath) -- ({\Rpath*sin(\angle)-\y}, \Rpath) (S) node[below left] {$S$};
    
    \draw[densely dotted] (-{\Rpath*sin(\angle)}, \Rpath+\y) -- ({\Rpath*sin(\angle)+1}, \Rpath+\y) (O) node[above right] {$O$};

    \draw[densely dotted] (F1)--(O) -- ++(3,0) coordinate(bob) ;

    \pic [draw, <-, "$\Tilde{\theta}$", angle eccentricity=1.1, angle radius=3.5cm] {angle = F1--O--bob};

    \draw[densely dotted, rotate around={{-\thetatilde - \deltac}:(F)} ](F) -- ++(2,0) coordinate(bob1);

    \pic [draw, <-, "$\delta$", angle eccentricity=1.2, angle radius=1.3cm] {angle = bob1--F--F1};

    \draw[densely dotted,rotate around={-\thetatilde:(T)}](T) -- ({-\Ts*cos(\thetatilde)+\Ty*sin(\thetatilde)+1.5}, {\Rpath+\y +\Ts *sin(\thetatilde)+\Ty*cos(\thetatilde)});

    \draw[densely dotted, rotate around={{90-\thetatilde}:(O)}] (O) -- (2,{\Rpath+\y});
    \draw[densely dotted] ({1.5*cos(90-\thetatilde)},{\Rpath+\y + 1.5*sin(90-\thetatilde)}) -- ({\wheelbase*cos(\thetatilde)+1.5*cos(90-\thetatilde)},{\Rpath+\y-\wheelbase*sin(\thetatilde) + 1.5*sin(90-\thetatilde)}) node[midway, above, black] {$L$} ;

    \draw[densely dotted, rotate around={{90-\thetatilde}:(F)} ](F) -- ({\wheelbase*cos(\thetatilde)+2},{\Rpath+\y-\wheelbase*sin(\thetatilde)});

    \draw[>=triangle 45, <->, line width=0.125mm, ForestGreen](T) -- ({90+\angle-2}:\Rpath) node[midway, left, black] {$y_T$} ;

    \draw[densely dotted, ForestGreen, shift = {(-1,0)}] ({90+\angle-2}:\Rpath) -- ++(\Rpath,0) ;

    \draw[>=triangle 45, <->, line width=0.125mm, ForestGreen, shift = {(-0.25,0)}] ({90+\angle-2}:\Rpath) -- ++(0,{\Rpath*(1-cos(\angle-2))}) node[midway, left, black] {$e$} ;

    \draw[>=triangle 45, <->, line width=0.125mm, shift = {(-0.5,0)}] (O) -- (S) node[midway, left, black] {$y$};

    \draw[densely dotted] (0, 0) -- (O) node[midway, right, black] {$\frac{1}{c(s)}$};
    
    \draw[densely dotted] (0, 0) -- ({90+\angle-2}:\Rpath) coordinate(bob4) node[midway, left, black] {$\frac{1}{c(s)}$};
    
    \pic [draw, <->, "$\xi$", angle eccentricity=1.2, angle radius=2.0cm] {angle=O--Origin--bob4};

    \end{scope}
\end{tikzpicture}

